Data-driven subgrouping of patient trajectories with chronic diseases: Evidence from low back pain

Clinical data informs the personalization of health care with a potential for more effective disease management. In practice, this is achieved by subgrouping, whereby clusters with similar patient characteristics are identified and then receive customized treatment plans with the goal of targeting subgroup-specific disease dynamics. In this paper, we propose a novel mixture hidden Markov model for subgrouping patient trajectories from chronic diseases. Our model is probabilistic and carefully designed to capture different trajectory phases of chronic diseases (i.e., "severe", "moderate", and "mild") through tailored latent states. We demonstrate our subgrouping framework based on a longitudinal study across 847 patients with non-specific low back pain. Here, our subgrouping framework identifies 8 subgroups. Further, we show that our subgrouping framework outperforms common baselines in terms of cluster validity indices. Finally, we discuss the applicability of the model to other chronic and long-lasting diseases.

==> CVI_comparison.tex <==
Latent class analysis (raw data)      & 7 & -0.15           & 1.77            &  8.91          & -0.12           & 3.47            &  11.89 \\
% \quad from \citet{Nielsen.2016}\\ 
Latent class analysis (two-stage process)      & 9 & -0.12           &  3.13   &  8.86  & \textbf{$-$0.09} &  3.79    & 12.06 \\ 
%\quad with two-stage process\\
   Clustering via $k$-means & 8 &  -0.11  & 1.21            & 9.92           &  -0.12  & 2.76          & 13.90  \\
   \midrule
 MHMM (ours)             & 8 & \textbf{$-$0.08} & \textbf{14.42} & \textbf{5.94} & -0.13           & \textbf{15.37} & \textbf{8.34} \\  
  

==> CVI_comparison_full.tex <==
% latex table generated in R 3.4.2 by xtable 1.8-2 package
% Thu Aug 09 08:23:09 2018
 MHMM~(Online) & 8        & \bfseries -0.08 & \bfseries 14.42 & 0.41 & \bfseries 0.08 & 0.23 & 0.36 & \itshape 5.82 & \bfseries 5.94 &\bfseries 0.47 & \bfseries 1.48 \\ 
 Latent class analysis& 7 & -0.15 & 1.77 & \itshape 0.42 & 0.06 &\itshape 0.27 &\bfseries 0.54 & \bfseries 4.18 & 8.91 & 0.50 & \itshape 2.33 \\
 \quad from \citep{Nielsen.2016}\\ 
Latent class analysis&9 & -0.12 & \itshape 3.13 & 0.38 & 0.08 & 0.26 & 0.44 & 7.37 & \itshape 8.86 & 0.50 & 2.66 \\ 
\quad with two-stage process\\
   Clustering via $k$-means& 8 & \itshape -0.11 & 1.21 & \bfseries 0.50 &\itshape 0.08 & \bfseries 0.35 & \itshape 0.52 & 8.73 & 9.92 & \itshape 0.51 & 2.75 \\
  \midrule
  \multicolumn{11}{l}{\textsc{Panel B: Disability trajectory}} \\
  \midrule 
 MHMM~(Online) 		  & 8 & -0.13 & \bfseries 15.37 & \bfseries 0.47 & \bfseries 0.08 & 0.28 & 0.46 & \itshape 6.99 & \bfseries 8.34 & \bfseries 0.47 & \bfseries 2.05 \\ 
 Latent class analysis& 7 & -0.12 & 3.47 & 0.40 & \itshape 0.06 & 0.27 & \itshape 0.47 & \bfseries 4.89 & 11.89 & 0.51 & 2.46 \\ 
 \quad from \citep{Nielsen.2016}\\ 
  Latent class analysis & 9 & \bfseries -0.09 & \itshape 3.79 & 0.47 & 0.05 & \bfseries  0.32 & \bfseries  0.50 & 7.43 & 12.06 & 0.50 & 2.61 \\ 
  \quad with two-stage process\\
  Clustering via $k$-means& 8 & \itshape -0.12 & 2.76 & \itshape 0.47 & 0.06 & \itshape 0.31 & 0.45 & 12.09 & 13.90 & 0.52 & 2.76 \\ 
  

==> cluster_description.tex <==
% latex table generated in R 3.4.2 by xtable 1.8-2 package
% Fri Aug 10 15:39:28 2018 # | Desc | #Patients | Male % | Age | BMI | Physical Work | Mean Pain | SD Pain | Mean Dis | SD Dis | pain 12m | Dis 12m
  1 & Severe fluctuating back pain & Mainly unstable phases with high pain and modest disability levels  &  18 & 55.56 & 41.20 & 25.64 & 44.44 & 5.59 & 1.98 & 1.75 & 2.22 & 5.33 & 26.09 \\ 
  2 & Severe back pain &Highly unstable phases involving recurrent and extent pain, as well as disability &  24 & 54.17 & 43.03 & 27.50 & 50.00 & 3.57 & 1.79 & 3.45 & 2.52 & 3.62 & 42.74 \\ 
  3 & Recovery & Mostly stable phases and hardly any activity limitations & 187 & 54.55 & 41.86 & 26.27 & 37.91 & 0.84 & 1.71 & 0.19 & 0.82 & 1.15 & 7.24 \\ 
  4 & Relapsing back pain&Low pain and disability levels, yet with frequent unstable phases for largely women with low BMI and frequent physical work &  14 & 35.71 & 42.79 & 24.63 & 50.00 & 0.92 & 1.43 & 2.02 & 2.99 & 1.25 & 18.48 \\ 
  5 & Early improvement back pain &Initial recovery but fluctuating condition with continuous unstable phases although low pain levels &  74 & 54.05 & 40.30 & 26.40 & 34.33 & 1.60 & 2.40 & 0.63 & 1.37 & 2.12 & 14.67 \\ 
  6 &Relapsing back pain &Only marginal improvement for female patients with low BMI and rare physical work &  13 & 38.46 & 45.86 & 24.00 & 7.69 & 1.63 & 1.14 & 0.95 & 1.63 & 1.50 & 18.84 \\ 
  7 & Persistent severe back pain & High pain and disability levels mostly affecting men with high BMI &  17 & 64.71 & 45.36 & 29.92 & 42.86 & 4.89 & 2.11 & 4.32 & 3.11 & 3.57 & 29.50 \\ 
  8 & Mild episodic & Prevalent recovery resulting in very stable phases, low pain, and modest disability levels &  75 & 52.00 & 45.70 & 26.09 & 36.49 & 0.93 & 1.72 & 0.57 & 1.66 & 1.24 & 9.39 \\ 
  

==> cluster_interpretation.tex <==
% latex table generated in R 3.4.2 by xtable 1.8-2 package
% Fri Oct 27 11:31:52 2017
1 & Severe back pain (highly unstable phases involving recurrent and extensive pain, as well as disability, with mostly females) &  16 & 37.50 & 48.05 & 28.17 & 43.75 & 3.74 & 3.30 & 2.77 & 2.98 & 2.09 & 27.67 \\ 

2 & Mild episodic (prevalent recovery from a largely work-induced condition for males, resulting in very stable phases, low pain and modest disability level) & 292 & 61.30 & 42.73 & 26.13 & 36.64  & 2.21 & 1.64 & 2.04  & 1.68 & 1.45 & 10.46 \\ 

3 & Recovery (with mostly stable phases and hardly any activity limitations)  &  26  & 42.31 & 45.01 & 23.05 & 15.38 & 2.40 & 1.92 & 2.07  & 2.02 & 1.25 & 8.87 \\ 

4 & Relapsing back pain (largely among females with marginal improvements, though low pain levels) &  13 & 23.07 & 44.78 & 24.54 & 46.15 & 2.75 & 1.58 & 2.23 & 1.54 & 2.58 & 18.12 \\ 

5 & Early improving back pain (initial recovery but fluctuating condition with continuous unstable phases for young patients with low BMI and rare physical work) &  20 & 35.00 & 29.71 & 27.85 & 15.00 & 3.62 & 2.20 & 2.78  & 2.03  & 2.81 & 18.21 \\ 

6 & Mild fluctuating back pain (short-term but fluctuating recovery, small improvements in pain, yet no clear tendency regarding patient outcomes)  &  41 & 36.59 & 43.35 & 28.87 & 46.34 & 3.39 & 2.00 & 2.66  & 1.98 & 3.13 & 21.83 \\ 

7 & Relapsing back pain (low pain and disability levels, yet with frequent unstable phases for largely females) &  11 & 18.18 & 41.75 & 25.37 & 45.45 & 2.32 & 1.42 & 1.91 & 1.21 & 0.90 & 12.17 \\ 

8 & Persistent severe back pain (affecting mostly males with high BMI) &   3 & 66.67 & 48.93 & 29.87 & 33.33  & 5.16 & 5.48 & 2.25 & 2.82  & 3.67 & 50.72 \\ 
  

==> number_of_clusters.tex <==
% latex table generated in R 3.4.2 by xtable 1.8-2 package
% Thu Aug 09 06:54:09 2018
 4 & 60173.54 & 61668.05 \\ 
%   & (2157.21) & (2157.32) & (2114.37) & (2120.10) \\ 
  5 & 59430.76 & 61273.29 \\ 
%   & (2122.48) & (2124.46) & (2083.53) & (2100.45) \\ 
  6 & 58397.57 & 60581.50 \\ 
%   & (2117.38) & (2191.28) & (2034.55) & (2067.17) \\ 
  7 & 58858.35 & 61045.49 \\ 
%   & (2072.24) & (2075.36) & (2017.79) & (2073.83) \\ 
  8 & 58004.53 & \bfseries 60454.25 \\ 
%   & (2063.31) & (2065.66) & (2011.05) & (2051.72) \\ 
  9 & 58664.46 & 61278.17 \\ 
 %  & (2025.48) & (2025.48) & (2025.48) & (2093.01) \\ 
  

==> number_of_states.tex <==
% latex table generated in R 3.4.2 by xtable 1.8-2 package
% Thu Aug 09 06:52:58 2018
 1 & 120541.19 & 121171.59 \\ 
%   & (3655.33) & (3655.07) & (3621.71) & (3551.72) \\ 
  2 & 74488.20 & 75341.76 \\ 
%   & (2879.13) & (2879.64) & (2862.44) & (2795.53) \\ 
  3 & 65776.12 & \bfseries 67066.60 \\ 
%   & (2433.58) & (2433.61) & (2416.65) & (2454.02) \\ 
  4 & 66523.64 & 67432.93 \\ 
%   & (2308.39) & (2308.56) & (2290.37) & (2302.31) \\ 
  

==> tpm_comparison.tex <==
% latex table generated in R 3.4.2 by xtable 1.8-2 package
% Fri Oct 27 10:38:43 2017
 Stable & 96.28 & 1.79 & 1.93 & 83.75 & 13.08 & 3.17 \\ 
   & (94.19,97.86) & (0.6,3.32) & (0.71,3.37) & (53.91,98.55) & (0.91,38.84) & (0.04,17.55) \\ 
  Unstable & 13.33 & 83.11 & 3.56 & 6.5 & 89.39 & 4.11 \\ 
   & (7.86,19.35) & (76.5,88.52) & (1.19,6.82) & (1.47,12.72) & (81.31,95.14) & (0.8,12.44) \\ 
  Acute & 12.08 & 16.74 & 71.19 & 0.44 & 3.63 & 95.93 \\ 
   & (5.41,19.45) & (9.87,25.97) & (63.29,79.3) & (0.01,1.6) & (1.35,6.82) & (92.42,98.44) \\ 
  
